$e^+ e^-$ angularity distributions at NNLL$^\prime$ accuracy

We present predictions for the $e^{+}e^{-}$ event shape angularities at NNLL$^{\prime}$ resummed and $\mathcal{O}(\alpha_s^{2})$ matched accuracy and compare them to LEP data at center-of-mass energies $Q=91.2$ GeV and $Q=197$ GeV. We perform the resummation within the framework of Soft-Collinear Effective Theory, and make use of recent results for the two-loop angularity soft function. We determine the remaining NNLL$^{\prime}$ and $\mathcal{O}(\alpha_s^2)$ ingredients from a fit to the EVENT2 generator, and implement a shape function with a renormalon-free gap parameter to model non-perturbative effects. Using values of the strong coupling $\alpha_s(m_Z)$ and the universal non-perturbative shift parameter $\Omega_1$ that are consistent with those obtained in previous fits to the thrust and $C$-parameter distributions, we find excellent agreement between our predictions and the LEP data for all angularities with $a\in[-1,0.5]$. This provides a robust test of the predictions of QCD, factorization, and the universal scaling of the non-perturbative shift across different angularities. Promisingly, our results indicate that current degeneracies in the $\{\alpha_s(m_Z),\Omega_1\}$ parameter space could be be alleviated upon fitting these parameters to experimental data for the angularity distributions.

==> Chapters/fitAPP.tex <==
\section{Fit parameters for $\cO(\as^2)$ remainder function}
\label{app:fit}

Here we present the results of fitting the $\tau_a<0.1$ region of the $\cO(\as^2)$ remainder function data obtained from \event, as described in \sec{remainder}. The \event\ predictions for the function $r_2(\tau_a)$ are fit to the functional form \eq{logfit}, with $a_{1,2,3},b_{2,3}$ the five free parameters in the fit, and $a_0$ determined by the constraint on the total area under $r_2$ obtained in \tab{d2}. The parameters we obtain are:
\begin{table}[h]
\begin{center}
\begin{tabular}{|c||c|c|c|c|c|c|c|}
\hline 
$a$ & $-1$ & $-0.75$ & $-0.5$ & $-0.25$ & 0 & 0.25 & 0.5 \\ \hline \hline
$a_1$ & $6212$ & $5401$ & $4328$ & $3526$ & $1475$ & $-209$ & $22756$  \\ \hline
$a_2$ & 1377 & 1210 &  986 & 803 & 343 & 50.8 & 6262  \\ \hline
$a_3$ & 94.4 & 82.5 &  67.3 & 54.2 & 23.5 & 14.0 & 512  \\ \hline
$b_2$ & -1680 & -1139 &  -518 & -491 & -25.4 & 793 & 4440  \\ \hline
$b_3$ & -2455 & -2098 &  -1619 & -1317 & -465 & 423 & -7037  \\ \hline\hline
$a_0$ & 5634 & 4694 &  3516 & 2884 & 1083 & -598 & 14658  \\ \hline
\end{tabular}
\end{center}
\caption{Results for the fit coefficients in \eq{logfit} obtained for the \event\ data displayed in \fig{r2all} and \fig{r2unc}. The parameter $a_0$ is fixed by the constraint that the area under the whole remainder function $r_2$ in \eq{r2joined} be equal to the values in \tab{d2}. The uncertainties on this fit are illustrated in \fig{r2unc} and are obtained from the \texttt{NonlinearModelFit} routine in Mathematica. The exact forms of these uncertainty functions are available upon request.}
\label{tab:fit}
\end{table}
